What Can You Learn from Your Muscles? Learning Visual Representation from Human Interactions

Learning effective representations of visual data that generalize to a variety of downstream tasks has been a long quest for computer vision. Most representation learning approaches rely solely on visual data such as images or videos. In this paper, we explore a novel approach, where we use human interaction and attention cues to investigate whether we can learn better representations compared to visual-only representations. For this study, we collect a dataset of human interactions capturing body part movements and gaze in their daily lives. Our experiments show that our "muscly-supervised" representation that encodes interaction and attention cues outperforms a visual-only state-of-the-art method MoCo (He et al.,2020), on a variety of target tasks: scene classification (semantic), action recognition (temporal), depth estimation (geometric), dynamics prediction (physics) and walkable surface estimation (affordance). Our code and dataset are available at: https://github.com/ehsanik/muscleTorch.

==> 00_main_cvpr.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% \usepackage{cvpr}
% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}

% %Added libraries
% \usepackage{comment}
% \usepackage{amsmath,amssymb} % define this before the line numbering.
% \usepackage{color}

% % \usepackage{ruler}
% % \usepackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}
% \usepackage{multirow}
% \usepackage{color}
% \usepackage{xspace}
% \usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}
% \usepackage{booktabs}
% \usepackage{makecell}

% \providecommand{\etal}{\textit{et al.}\xspace}
% % \providecommand{\datasetname}{HumanData}
% % \providecommand{\ourmethod}{Muscly}
% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% \providecommand{\kiana}[1]{{\protect\color{green}{\bf [Kiana: #1]}}}
% \providecommand{\todo}[1]{{\protect\color{red}{\bf [TODO: #1]}}}


% % Include other packages here, before hyperref.

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false]{hyperref}

% \cvprfinalcopy % *** Uncomment this line for the final submission

% \def\cvprPaperID{****} % *** Enter the CVPR Paper ID here
% \def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% % Pages are numbered in submission mode, and unnumbered in camera-ready
% \ifcvprfinal\pagestyle{empty}\fi
% \begin{document}

% %%%%%%%%% TITLE
% \title{
% % What Can You Learn From Your Muscles?
% Learning Visual Representation from Joint Movements and Gaze
% }

% \author{Kiana Ehsani$^1$ \and
% Daniel Gordon$^1$\and
% Thomas Nguyen$^1$\and
% Roozbeh Mottaghi$^2$\and
% Ali Farhadi$^1$\\
% $^1$ University of Washington, $^2$ Allen Institute for AI
% }
% %
% % \authorrunning{F. Author et al.}
% % First names are abbreviated in the running head.
% % If there are more than two authors, 'et al.' is used.
% %
% % \institute{University of Washington %\email{kianae@cs.washington.edu}
% % \and
% % Allen Institute for AI
% % }


% \maketitle
% %\thispagestyle{empty}


% %%%%%%%%% ABSTRACT

% \begin{abstract}
% \input{01_abstract}
% \todo{abstract}
% \end{abstract}

% \todo{spell check stuff}

% \begin{figure*}[tp]
%     \centering
%     \includegraphics[width=40pc]{figs/human_teaser.pdf}
%     \caption{We propose ``Muscly Supervised" representation learning, where the idea is to use body part movement and gaze cues in addition to visual cues. We mount movement sensors on the body parts of different subjects to capture their movements. We also mount a camera on the subjects' head and capture first-person videos along with the gaze information, which is obtained by a pair of eye-tracking glasses. We use the learned representation on several different types of tasks (semantic, temporal, geometric, physics and affordance prediction) and show consistent improvements across all tasks compared to state-of-the-art unsupervised techniques. The red circle in the image shows the location of the gaze, and the red circle on the human icon shows the active sensor in those particular frames.}
%     \label{fig:teaser}
% \end{figure*}
% \input{01_intro_distillation}
% \input{02_related}
% \input{03_dataset}
% \input{04_approach}
% \input{05_experiment}
% \input{06_discussion}

% {\small 
% \textbf{Acknowledgments.} \todo{add fundings }
% }

% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \end{document}


==> abstract_roozbeh.tex <==
Recent self-supervised and unsupervised representation learning approaches are typically trained with visual data available in large-scale datasets. These approaches have achieved impressive classification performance that is close to supervised training. In this paper, we investigate whether additional cues such as human body part movements and human gaze, which are highly correlated with the visual signal, can lead to learning better representations that generalize across different tasks. For this purpose, we collect an unlabeled dataset of about \todo{XX} million images with the corresponding body part movements and gaze information during the daily activities of people. Our experiments show that models trained using these additional cues generalize better to a variety of target tasks compared to the models that rely only on the visual cues. More specifically, when trained with the same number of parameters and the same data, our learned representation outperforms a recent state-of-the-art approach that is trained on only the visual cues on five different target tasks: scene classification, action recognition, depth estimation, dynamics prediction and walkable surface estimation.   


==> boring_intro.tex <==

\section{Introduction}

Representation learning has recently attracted many researchers in the field. There are several approaches for tackling this problem. Traditional supervised learning methods train their models on a predefined task and collect a dataset with labels addressing that problem.\cite{imagenet} Recently self-supervised methods propose training without semantic labels on the same datsaets.

The common property among all these approaches is using a proxy task to train the representations , eg. predicting imagenet clsases\cite{}, colorizing grayscale images\cite{} and contrasting different augmentations of images\cite{}. These methods are shown to be capable of learning representations that are generalizable to variety of end tasks. These proxy tasks mostly lie within the following two categories, 1) they directly use semantic labels (eg. imagenet pretrained models), or 2) they use the data that is organized and structured in a semantic way (eg. moco unsupervised training on imagenet images). 

However, there is a third category of non-semantic proxy objectives which use low-level tasks such as colorization, optical flow and reconstruction \cite{}. In this paper we introduce another approach in this category. Inspired by the way animals learn and act in the real world and motivated by recent movement toward embodied visual intelligence, we want to directly learn from intelligent agents. 

Instead of using human supervision to go to semantic space, we argue that we can approach the problem by directly learning from their actions. These actions cover a wide range of tasks including semantic and non semantic cues. These cues come together in one of our basic properties, our muscles. When we observe and interact with the visual world, one way to measure our actions is by quantifying the movements in the muscles, changes in the center of focus, heart rate, etc. \todo{maybe an example}

% , which impact our movements and our gaze. 
% When we observe the visual world, one measurable acion we do is to move muscles 

In this paper we learn our representations from human muscle movements and show that this representation is richer than just training on visual features and generalizes well to different domains of semantic and low level tasks. Our contribution is threefold:

1) We introduce a new dataset of ego-centric videos with the corresponding movement and gaze of the performer. We collect 77 hours of video that is captured from 35 people over 4 months, which amounts to 16 million frames in indoor and outdoor scenes. A wide range of activities such as driving, shopping, playing ping pong have been covered in the dataset. This dataset can be beneficial for tasks other than representation learning as well. 

2) We train a model to predict gaze and body part movements from the ego-centric videos, and we show that encoding gaze, muscle movements and visual cues in this learned representation makes it generalizable to a variety of target tasks: semantic (scene classification), temporal (action recognition), geometric (depth estimation), physics (dynamics prediction) and affordance-based (walkable surface estimation).

3) Our approach outperforms MoCo \cite{he2019momentum}, a strong unsupervised representation learning technique, on all five target tasks when it is trained on the same visual data. We conclude that movement and gaze information helps learn a better representation compared to a visual-only model. 

==> intro_roozbeh.tex <==
\section{Introductions}

Learning compact representations for image contents that can generalize to multiple visual tasks has been a long quest of computer vision. The common practice in the deep learning era is to pre-train a neural network using a large-scale annotated dataset \cite{Deng2009ImageNetAL,wslimageseccv2018,openimages} and fine-tune the network or some part of it to adapt it to a new target task \cite{Zamir_2018_CVPR}. A major issue is that curating such large datasets is costly and time-consuming, and this way of training a network is different from how humans learn visual representations. Self-supervised and unsupervised methods (e.g., \cite{Wang2017TransitiveIF,hjelm2018learning,wu2018unsupervised,he2019momentum}) have been explored to mitigate the need for such curated datasets.

Unsupervised and self-supervised approaches have recently achieved a classification accuracy close to supervised training. However, there is an important question that is yet to be answered. Can we learn better representations using other signals that are correlated with the visual signal? For example, can we learn a better visual representation by using the information encoded in body part movements? or can attention (gaze) be used as an additional cue for learning better representations? 

%Second, do these unsupervised methods work on unconstrained data? or do they learn a generalizable representation only if they are trained on cleaned up and manually annotated datasets such as ImageNet? It should be noted that these high-performing methods \cite{} do not use the class labels for training, but the training is performed on these curated data, where there is a balanced set of images for each category and there is no noise in the data.

This paper is an initial attempt to answer this question. We propose a ``muscly-supervised" approach to learn visual representations. Our idea is to augment visual representation learning by body part movements and gaze corresponding to the visual observation. More specifically, we propose an approach that predicts body part movements and gaze from a sequence of observed images. For this purpose, in addition to a camera, we mount a set of sensors that capture body part and gaze movements on different people and record this information during their daily activities. We train our model in a self-supervised way using losses that are defined based on the visual and movement information. We refer to our approach as ``muscly-supervised" since the movements of the body parts and the gaze are caused by the muscles. 

We introduce a new dataset that includes 77 hours of video that is captured from 35 people over 4 months, which amounts to 16 million frames in indoor and outdoor scenes. A wide range of daily activities such as driving, shopping, playing ping pong have been covered in the dataset. There was no constraints on the actions and the subjects performed their routine daily activities. 

We learn a representation using visual, movement and gaze cues provided by the dataset. To evaluate the learned representation, we test it on a variety of target tasks: semantic (scene classification), temporal (action recognition), geometric (depth estimation), physics (dynamics prediction) and affordance-based (walkable surface estimation).

We show that our representation learning approach outperforms MoCo  \cite{he2019momentum} style of training, which is a state-of-the-art unsupervised representation learning on all five target tasks, when it is trained on the same visual data. This means movement and gaze information can help learning a better representation compared to a visual-only model. We also show that not all body parts or gaze are required for a task. Some tasks might benefit more from certain movements. For example, the visual and gaze features provide better performance on the target task of walkable surface estimation compared to the case that we use all information. 


% \kiana{Why not moco? imagenet and instagram are both biased, object in the center of image, blah blah}

% this paper showed imagenet is biased~\cite{geirhos2018imagenet}

\begin{figure}[tp]
    \centering
    \includegraphics[width=29pc]{figs/human_teaser.pdf}
    \caption{We propose ``Muscly Supervised" representation learning, where the idea is to use body part movement and gaze cues in addition to visual cues. We mount movement sensors on the body parts of different subjects to capture their movements. We also mount a camera on the subjects' head and capture first-person videos along with the gaze information, which is obtained by a pair of eye-tracking glasses. We use the learned representation on several different types of tasks (semantic, temporal, geometric, physics and affordance prediction) and show consistent improvements across all tasks compared to state-of-the-art unsupervised representation learning methods that similar to us do not use any manual annotation, but rely on only visual cues. The red circle in the image shows the location of the gaze, and the red circle on the human icon shows the active sensor in those particular frames.}
    \label{fig:teaser}
\end{figure}

==> old_01_intro_distillation.tex <==
\section{Introduction}

Encoding visual information from pixel space to a lower dimensional vector is the core element of most modern deep learning based solutions to computer vision. Researchers have developed a rich set of algorithms and techniques to enable learning these encodings. Typically, networks are explicitly trained to directly map visual inputs to a final label space using end-to-end training. The embeddings learned this way does not necessarily generalize to other tasks. Instead of only using the final target labels, researchers have used proxy tasks and learned to predict the proxy labels. For example, when labeled data is sparse, predicting ImageNet labels has been extensively used as a proxy task to learn representations for other tasks. 

Several other proxy tasks have been explored to learn visual representations. Some use semantic labels (e.g., image classification~\cite{he2016deep}, captioning~\cite{li2019visualbert}) while others benefit from non-semantic cues (e.g., colorization~\cite{zhang2016colorful}, jigsaw puzzles~\cite{noroozi2016unsupervised}, etc). Researchers have also used the output of another network as proxy labels to learn good representations. A student network learns to predict the outcome of a teacher network with the goal of transferring the knowledge learned by the teacher to the student \cite{yan2019clusterfit,bagherinezhad2018label,hinton2015distilling}. 

In this paper, we further explore the idea of using a teacher to learn good visual embeddings. We ask the following question: what is the best visual-encoding teacher to learn from? Literature suggests using robust\cite{yalniz2019billion}, high capacity \cite{yalniz2019billion}, large\cite{xie2019self} teachers. In this paper, we take an orthogonal approach; \textit{what if we can use human brain as a teacher?}

The human brain is far too complex to be understood by modern science, and measuring the outcome of the ``brain network", if at all  possible, is way outside of our domain of expertise. However, a few steps removed from brain signals may still yield meaningful proxies. In this paper, we argue that looking at the muscular reactions to visual stimuli provides signals that serve as a weak proxy for the output of the ``brain network.'' When we observe the visual world, parts of our visual understanding will be reflected by our muscle activations. For example, our heart pumps faster when we see something exciting, our eye muscles contract to focus on the target, and  we move our legs to run towards it.

To study what we can learn from muscular activations, we attach sensors to humans and see how they react to visual events in their daily lives. More specifically, we record major limb movements that we can measure with common Inertial Movement Units (IMUs). In addition, we record gaze to monitor muscle movements in eyes. Figure~\ref{fig:dataset} shows an example of our setup. We recorded 77 hours of ego-centric videos in their daily lives for 35 individuals, along with their gaze and muscle movements. 
%Note that these measurements are not the most accurate way to record muscle activations, and the visual stimuli exposed to our subjects are not isolated in controlled settings. 
%However, our design decisions ensure the minimum scale necessary to validate our hypothesis rather than being clinically accurate in our measurements with the cost of small scale data.  

Our experimental results show that \textit{there is a lot to be learned from your muscles}. In particular, our representation learned by predicting gaze and body part movements generalizes to a variety of target tasks: scene classification (semantic), action recognition (temporal), depth estimation (geometric), dynamics prediction (physics) and walkable surface estimation (affordance-based). The representation learned via muscles can also improve upon the representations learned purely from visual cues  (e.g. MoCo\cite{he2019momentum}). It is interesting to note that different tasks benefit from different muscular information. For example, limb movements are more beneficial to low-level tasks while attention cues are more helpful for more semantic tasks.  
% We observe that the low-level task of depth estimation depends 
%For example, that movement cues seem more helpful for low-level tasks such as depth estimation, in contrast to the semantic tasks such as walkable surface estimation which benefits most from attention cues.

% It is also interesting to see that, the representaion learned by muscles use XXX for task Y, etc, etc. 

% \todo{if we end up with this intro we need to rewrite related works.}



==> old_01_intro_kiana.tex <==
\section{Introduction}

Learning a visual representation is studied extensively from a variety of perspectives, from supervised learning using manually annotated datasets~\cite{Deng2009ImageNetAL,wslimageseccv2018,openimages} to learning low-level tasks without direct supervision~\cite{zhang2016colorful}. The common aim is to learn a rich embedding that can easily generalize to new tasks. These approaches rely on semantic supervision either in the form of explicit labels or for the construction of the dataset itself (e.g. training unsupervised on images from Imagenet or searched terms on the internet). Although these methods continue to shape the field, finding the optimal regime for learning visual features is still an open research problem.


Humans are visually intelligent by nature, yet they do not need to look at distorted, augmented images with unorthodox object shapes to learn about the visual world. They learn instead through interaction with the environment.


Humans interact with the world in a variety of different ways, resulting in a better understanding of the environment. As an example, our visual understanding of the world and our movements are inextricably linked. We react to a ball thrown at us by moving our hand to catch it. Moreover, we use our eye muscles to concentrate on a specific region of a scene to extract more details from our region of interest. Even when we walk down the street, we subconsciously avoid hitting people or tripping. Labeling ``why'' someone does a certain actions may be impossible, so instead, in this work, we observe ``what'' people do when going about their daily lives.

In this paper we focus on the non-semantic task of encoding these muscular cues in the visual features. By doing so we hope to learn from the human understanding of the visual world. 
People's movements and attention provide a rich underlying signal to learn generalizable representations. 
More specifically, we propose an approach that predicts body part movements and gaze from a sequence of observed images. We introduce a new dataset including 77 hours of video captured from 35 people over 4 months, which amounts to 16 million frames in indoor and outdoor scenes. The dataset covers a wide range of activities such as driving, shopping, and playing ping pong. The subjects performed their routine daily activities and there are no constraints on the actions. We anticipate that this dataset will be beneficial for tasks other than representation learning. Refer to supplementary material for sample videos of our dataset.

We train our model in a \todo{not self}self-supervised way using the visual and movement information. We refer to our approach as ``muscly-supervised"\todo{replace} since the movements of the body parts and the gaze are driven by muscles. 
We evaluate the learned representations by testing them on a variety of target tasks: semantic (scene classification), temporal (action recognition), geometric (depth estimation), physics (dynamics prediction) and affordance-based (walkable surface estimation).

Our approach outperforms MoCo \cite{he2019momentum}, a strong unsupervised representation learning technique, on all five target tasks when it is trained on the same visual data. We conclude that movement and gaze information helps learn a better representation compared to a visual-only model. 



==> old_intro.tex <==
\section{Introductions}

Learning low-dimensional representations for image contents that can generalize to multiple visual tasks has been a long quest of computer vision. The common practice in the deep learning era is to pre-train a neural network using a large-scale annotated dataset \cite{Deng2009ImageNetAL,wslimageseccv2018,openimages} and fine-tune the network or some part of it to adapt it to a new target task \cite{Zamir_2018_CVPR}. A major issue is that curating such large datasets is quite costly and time-consuming, and this way of training a network is very different from how humans learn visual representations. Self-supervised and unsupervised methods (e.g., \cite{Wang2017TransitiveIF,hjelm2018learning,wu2018unsupervised,he2019momentum}) have been explored to mitigate the need for such curated datasets.

Unsupervised and self-supervised approaches have recently achieved a classification accuracy close to supervised training. However, there is an important question that is yet to be answered. Can we learn better representations using other signals that are correlated with the visual signal? For example, can we learn a better visual representation by using the information encoded in body part movements? or can attention (gaze) be used as an additional cue for learning better representations? 


This paper is an initial attempt to answer this question. We propose a ``muscly-supervised" approach to learn visual representations. Our idea is to augment visual representation learning by body part movements and gaze corresponding to the visual observation. More specifically, we propose an approach that predicts body part movements and gaze from a sequence of observed images. For this purpose, in addition to a camera, we mount a set of sensors that capture body part and gaze movements on different people and record this information during their daily activities. We train our model in a self-supervised way using losses that are defined based on the visual and movement information. We refer to our approach as ``muscly-supervised" since the movements of the body parts and the gaze are caused by the muscles. 

We introduce a new dataset that includes 77 hours of video that is captured from 35 people over 4 months, which amounts to 16 million frames in indoor and outdoor scenes. A wide range of activities such as driving, shopping, playing ping pong have been covered in the dataset. There was no constraints on the actions and the subjects performed their routine daily activities. This dataset can be beneficial for tasks other than representation learning as well. 

To evaluate the learned representation, we tested it on a variety of target tasks: semantic (scene classification), temporal (action recognition), geometric (depth estimation), physics (dynamics prediction) and affordance-based (walkable surface estimation).

Our experiments result in interesting findings. We show that our representation learning approach outperforms MoCo \cite{he2019momentum}, which is a state-of-the-art unsupervised representation learning on all five target tasks, when it is trained on the same visual data. This means movement and gaze information can help learning a better representation compared to a visual-only model. We also show that not all body parts or gaze are required for a task. Some tasks might benefit more from certain movements. For example, the visual and gaze features provide better performance on the target task of walkable surface estimation compared to the case that we use all information. 


% \kiana{Why not moco? imagenet and instagram are both biased, object in the center of image, blah blah}

% this paper showed imagenet is biased~\cite{geirhos2018imagenet}

\begin{figure}[tp]
    \centering
    \includegraphics[width=29pc]{figs/human_teaser.pdf}
    \caption{We propose ``Muscly Supervised" representation learning, where the idea is to use body part movement and gaze cues in addition to visual cues. We mount movement sensors on the body parts of different subjects to capture their movements. We also mount a camera on the subjects' head and capture first-person videos along with the gaze information, which is obtained by a pair of eye-tracking glasses. We use the learned representation on several different types of tasks (semantic, temporal, geometric, physics and affordance prediction) and show consistent improvements across all tasks compared to state-of-the-art unsupervised representation learning methods that similar to us do not use any manual annotation, but rely on only visual cues. The red circle in the image shows the location of the gaze, and the red circle on the human icon shows the active sensor in those particular frames.}
    \label{fig:teaser}
\end{figure}

==> v1_intro.tex <==
\section{Introduction}
\vspace{-0.2cm}
% Comments:
% {
% The embeddings learned this way does not necessarily generalize to other tasks --> this is not necessarily true. they generalize to some extent
% used "encoding" and "embedding" for the same thing in the first paragraph}

% \kiana{representation learning is popular, people trained on imagenet, imagenet requires data, unsupervised representation learning arose}

Encoding visual information from pixel space to a lower-dimensional vector is the core element of most modern deep learning-based solutions to computer vision. A rich set of algorithms and architectures have been developed to enable learning these encodings. A common practice in computer vision is to explicitly train the networks to map visual inputs to a curated label space. For example, a neural network is pre-trained using a large-scale annotated classification dataset \citep{Deng2009ImageNetAL,openimages} and the entire network or part of it is fine-tuned to a new target task \citep{goyal2019scaling,Zamir_2018_CVPR}.

%is to pre-train a neural network using 

%Typically,  
 %A major issue is that curating such large datasets is costly and time-consuming. Self-supervised and unsupervised methods (e.g., \citep{Wang2017TransitiveIF,hjelm2018learning,wu2018unsupervised,he2019momentum}) have been explored to mitigate the need for such curated datasets.


% \kiana{contrastive learning is the most popular unsupervised rep learning but it's different from how humans learn, we learn from interaction}
In recent years, weakly supervised and unsupervised representation learning approaches (e.g., \cite{Mahajan2018ExploringTL,he2019momentum,chen2020simple}) have been proposed to mitigate the need for supervision. The most successful ones are contrastive learning-based approaches such as \citep{he2019momentum,chen2020simple} and they have shown remarkable results on target tasks such as image classification and object detection. Despite their success and impact, there are two primary caveats: (1) These self-supervised methods are still trained on ImageNet or similar datasets, which are fairly cleaned up and/or  include a pre-specified set of object categories. (2) This way of training i.e. contrasting two augmented patches of the same image, is far from how humans learn to perceive the visual world. A vast majority of our visual understanding is shaped by our interactions and our observations from others interacting with their environments. By learning how to move the joints to walk and crawl, infants can significantly enhance their perception and cognition~\citep{motordevelopment}. Moreover, by observing another person interact with the environment humans obtain visual and physical perception of the world~\citep{bandura77}. 


% We touch objects to understand their shapes, we blah blah\todo{adding psychology developmental reference}. \todo{This paragraph needs more examples I think to prove the point better.}
% Baillargeon, R. (1998) 'Infants' understanding of the physical world', Advances in psychological science, 2, pp. 503–529.
% Adolph, K. E. and Robinson, S. R. (2015) 'Motor development.', Handbook of child psychology and developmental science, pp. 114–157. doi: 10.1002/9780470147658.chpsy0204.
%Page 145
% Needham, A. and Baillargeon, R. (1998) 'Effects of prior experience on 4.5-month-old infants' object segregation', Infant Behavior and Development, 21(1), pp. 1–24. doi: 10.1016/S0163-6383(98)90052-2.
% Ramsey, R. and Hamilton, A. (2012) 'How does your own knowledge influence the perception of another person's action in the human brain?', pp. 1–29.
% Markson, L. and Spelke, E. S. (2006) 'Infants' rapid learning about self-propelled objects', Infancy, 9(1), pp. 45–71. doi: 10.1207/s15327078in0901_3.
% Himmler, B. T., Pellis, S. M. and Kolb, B. (2013) 'Juvenile play experience primes neurons in the medial prefrontal cortex to be more responsive to later experiences', Neuroscience Letters. Elsevier Ireland Ltd, 556, pp. 42–45. doi: 10.1016/j.neulet.2013.09.061.
% Sim, Z. L., Mahal, K. K. and Xu, F. (2017) 'Learning about causal systems through play', Proceedings of the 39th Annual Conference of the Cognitive Science Society, pp. 1078–1083.
% The first Baillargeon reference is just a good primer on how we test the cognitive abilities of infants and not strictly relevant to the question at hand.

% \kiana{what do we mean by interaction? body part movement, we need to collect a dataset for it}
% To investigate this idea, we first need to define interaction. 
The question we investigate in this paper is, ``can we learn a rich generalizable visual representation by encoding human interactions into our visual features?". In this work, we consider the movement of human body parts and center of attention (gaze) as an indicator of their interactions with the environment and propose an approach for incorporating interaction information into the representation learning process. %\todo{for roozbeh, how is it done?}

To study what we can learn from interaction, we attach sensors to humans and see how they react to visual events in their daily lives. More specifically, we record major limb movements by Inertial Movement Units (IMUs). In addition, we record gaze to monitor the center of attention. We introduce a new dataset of more than 4,500 minutes of interaction by 35 participants engaging in everyday scenarios with their corresponding body part movements and center of attention. There are no constraints on the actions, and no manual annotations or labels are provided. %Furthermore, we train a model that predicts the human movements and attention based on the visual observation. 

%To capture human interactions,  

% \kiana{what do our results show?}
Our experiments show that the representation we learn by predicting gaze and body movements in addition to the visual cues outperforms the visual-only baseline on a diverse set of target tasks (Figure~\ref{fig:teaser}): semantic (scene classification), temporal (action recognition), geometric (depth estimation), physics (dynamics prediction) and affordance-based (walkable surface estimation). This shows movement and gaze information can help learning a better representation compared to a visual-only model. We also show that not all body parts or gaze are required for a task. Some tasks might benefit more from certain cues. For example, the visual and gaze features provide better performance on the target task of walkable surface estimation compared to the movement cues. 

% \kiana{summary of contributions}
%In summary, the contribution of this work is threefold: a) we show that our learned representation from human's interactions with the visual world improves MoCo \citep{he2019momentum}, which is a state-of-the-art unsupervised representation learning, on a variety of target tasks when it is trained on the same visual data, b) we investigate the importance of different interaction cues, joint and gaze, on the performance of end tasks, and c) we introduce a rich dataset of ego-centric videos of subjects performing their routine activities with their corresponding audio, absolute joint angles, movements and gaze tracker, which will be released to public for further research.

